Leveraging Uncertainty Estimates To Improve Classifier Performance

Binary classification involves predicting the label of an instance based on whether the model score for the positive class exceeds a threshold chosen based on the application requirements (e.g., maximizing recall for a precision bound). However, model scores are often not aligned with the true positivity rate. This is especially true when the training involves a differential sampling across classes or there is distributional drift between train and test settings. In this paper, we provide theoretical analysis and empirical evidence of the dependence of model score estimation bias on both uncertainty and score itself. Further, we formulate the decision boundary selection in terms of both model score and uncertainty, prove that it is NP-hard, and present algorithms based on dynamic programming and isotonic regression. Evaluation of the proposed algorithms on three real-world datasets yield 25%-40% gain in recall at high precision bounds over the traditional approach of using model score alone, highlighting the benefits of leveraging uncertainty.

==> sections/analysis2.tex <==

To understand the behavior of estimation bias, we consider a representative data generation scenario  and then analyse the dependence of estimation bias on uncertainty for this scenario with a focus on Posterior Networks though one can generalize it to other uncertainty modeling approaches. 

\noindent{\bf Notation.} Let $\x$ denote an input point and $y$ the corresponding target label that takes values from the set of class labels $\cC =\{ 0, 1 \}$ with $c$ denoting the index over the labels. 
%Further, let  $\cD_{train}$ denote the data used for training, $\theta, \phi$ the model 
% parameters and $\z= \z(\x)$ the output representation from the model. 
We use $\pr(\cdot)$ to denote probability and $[i]_{lb}^{ub}$ to denote an index  iterating over integers in $\{lb, \cdots, ub\}$.


\noindent{\bf 3.1 Background: Posterior Network}
Posterior Network \citep{posterior_network}  estimates a closed-form posterior distribution over predicted class probabilities for any new input sample via density estimation as described  in Appendix \ref{appendix:posterior}.  For binary classification, the posterior distribution at  $\x$ is a Beta distribution with parameters estimated by combining the model prior with pseudo-counts generated based on the learned normalized densities and observed class counts. Specifically,  denoting the model prior and observed counts for the class $c \in \cC$ by $\beta_c^{P}$ and $N_c$, the posterior distribution of the predicted class probabilities (a.k.a  epistemic distribution) at $\x$ is given by 
\begin{equation}
q(\x)=  \mbox{Beta}( \alpha_1(\x),\alpha_0(\x) )
\end{equation}
where $\alpha_c(\x)= \beta_c^{P} + \beta_c(\x)$   and $\beta_c(\x) = N_c \pr(\z(\x) | c; \phi),~ \forall c  \in {\cal C}$.  Model score $S^{model}(\x)$ for positive class is given by 
\begin{equation}
S^{model}(\x) =  \frac{ \beta_1^{P} +  \beta_1(\x)} { \sum_{c=0,1} [\beta_c^{P} +  \beta_c(\x)]}  =  \frac{\alpha_1(\x)}{\alpha_1(\x) + \alpha_0(\x)} 
\label{eqn:smodel}
\end{equation}
Uncertainty $u(\x)$ for $\x$ is given by the entropy of the epistemic distribution 
$H(q(\x))$.  Since $q(\x)$ is Beta distribution, for same score, i.e., $\alpha_1(\x)$/$\alpha_0(\x)$, uncertainty is higher when $\sum_{c \in \cC} \alpha_c(\x)$ is lower.

\noindent{\bf 3.2 Analysis of Estimation Bias}: For an input point $\x$, let $S^{true}(x), S^{train}(x),  S^{test}(x), S^{model}(x)$ denote the true positivity, empirical positivity in the train and test sets, and the model score  
respectively.  Assuming the train and test sets are drawn from the same underlying distribution with possible differential sampling across the classes, these variables are dependent on each other as shown in Fig. \ref{fig:dependencies}.  We consider the following generation mechanism where the true positivity rate is sampled from a global beta prior, i.e., 
$S^{true}(x) \sim Beta(\beta_1^T, \beta_0^T) $.  The labels $y(\x)$ in the test set are generated via Bernoulli distribution centered at $S^{true}(x)$. In case of the train set, we assume that the negative class is sampled at the rate  $\frac{1}{\tau}$\footnote{$\tau >1 $  corresponds to undersampled negatives while $\tau <1$ corresponds to oversampled negative class.} compared to positive class, i.e., labels can be viewed to be generated from a Bernoulli centered around $\frac{\tau S^{true}(x)} {\tau S^{true}(x) + (1-S^{true}(x)) }$. 
For this scenario,  the expected true and test positivity conditioned on the model score and uncertainty are given by Theorem \ref{hm:bias}.
 \todo{SM: mention proofs are in appendix}
\begin{theorem} 
\label{hm:bias}
For the case where the negative class is  undersampled at the rate $\frac{1}{\tau}$ during training, the expected test and true positivity rate conditioned on the model score for  positive class from Posterior Network,  $S^{model}(x) =s$ are equal and  given by 
$$ E [ S^{true}(x) | S^{model}(x) = s ] = E [ S^{test}(x) | S^{model}(x) = s ] = 
 \frac{e(s) +f(s)\gamma(\x)}{g(s)+h(s)\gamma(\x)}, $$ 
% where
 \begin{itemize}
\item  $\omega =\frac{\beta_1^{P}}{\beta_1^{P} + \beta_0^{P}}$ and $\xi =\frac{\beta_1^{T}}{\beta_1^{T} + \beta_0^{T}}$  are the positive prior ratios,  
\item $\gamma(\x) = \underbrace{\frac{\beta_1^{P} + \beta_0^{P}} {\beta_1(x) + \beta_0(x)}}_{\text{model-priors : evidence}}  ;$   $~~\nu = \underbrace{ \frac{\beta_1^{T} + \beta_0^{T}} {\beta_1^P + \beta_0^P}}_{\text{true-priors : model-priors}}$
\item $e(s) =s $; $~~f(s) = s + \xi\nu -\omega $; $~~g(s) = \tau- (\tau -1)s  $; $~~h(s) =\tau\nu - (\tau-1)(s+ \xi\nu -\omega) $
\end{itemize}
\label{thm:bias}
\vspace{-2mm}
\end{theorem}
% \proofsketch
% Given $S^{model}(x)$ and $\gamma(x)$, the train positivity rate $S^{emp-train}(x)$
% can be estimated from Eqn. \ref{eqn:smodel}.  Observing that train samples are generated from a Bernoulli distribution with mean dependent on $S^{true}(x)$, we use Bayes rule to estimate the expected true positivity rate conditioned on the train positivity and model score. 
% Since the test samples are generated from a Bernoulli centered at $S^{true}(x)$ and the test positivity rate $S^{emp-test}$ is conditionally independent of the $S^{emp-train}$  given $S^{true}(x)$, the expected test positivity rate is the same as that of the true positivity. 
% Further details are presented in Appendix \ref{proof}.
\qed

\noindent {\bf Interpretation of $\gamma(\x)$.}  Note that $\sum_c {\alpha_c(\x)}  =  [\sum_c \beta^{prior}_c ] (1 + \frac{1}{\gamma(\x)})$.   For a fixed score,  $\sum_c{\alpha_c(\x)}$  is inversely correlated to uncertainty $H(q(\x))$, hence $\gamma(\x)$ is positively correlated with $H(q(\x))$.

\noindent  {\bf No differential sampling $(\tau =1)$}.
%In this case, expected test positivity equals $\frac{s + (s + \xi\nu - \omega)\gamma(x)}{ 1 + \nu\gamma(x)}.$ 
Since the model scores are estimated by combining the model priors and the evidence,  $S^{model}(x)$  differs from the empirical positivity rate in the direction of the model prior ratio $\omega$. On the other hand, the expected true/test positivity rate differs from the empirical positivity rate in the direction of the true class prior ratio $\xi$. When the model prior matches the true class prior both on the positive class ratio and magnitude,$i.e., \nu=1, \xi=\omega$, then there is no estimation bias. In practice, model priors are often choosen to have low magnitude and the estimation bias is primarily influenced by global prior ratio with  overestimation (i.e., expected test positivity < model score) in the higher score range $(\xi < S^{model}(\x))$ and the opposite is true when $(\xi > S^{model}(\x))$.  The extent of the bias depends on the relative strengths of the priors  and the evidence  denoted by $\gamma(\x)$, which is correlated with uncertainty. 

\noindent  {\bf General case $(\tau > 1)$.} Here the expected behavior is affected not only by the interplay of the model prior, true class prior and evidence as in case of $\tau=1$, but also the differential sampling.  While the first component is similar to the case $\tau=1$ and results in over and under estimation in different score regions, the second component results in  overestimation across the entire score range with the extent of bias increasing with $\tau$.  Fig. ~\ref{fig:biasanalysis} shows the expected positivity rate for a few different choices of $\gamma(\x)$ and a fixed choice of $\omega=0.5$ and $\tau=10$. We validate this behavior by comparison with empirical observations in Section \ref{sec:experiment}. 
%SM: More details on the trends in the Appendix [Optional for AMLC]


\begin{wrapfigure}{l}{0.5\textwidth}
% \hfill
\subfigure[]{\includegraphics[width=0.47\linewidth]{images/teaser/simul/Picture 21.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.4\linewidth]{images/teaser/simul/Picture 22.pdf}}
% \hfill
\vspace{-3mm}
\caption{\footnotesize (a) Positivity rate vs. model score for $\omega=0.5,~\tau=10$ and a few choices of $\gamma(\x)$ as per Theorem \ref{thm:bias}. (b) Positivity rate for different model 
score and uncertainty ranges on synthetic data.}
\label{fig:biasanalysis}
\vspace{-5mm}
\end{wrapfigure}

The primary takeaway from Theorem \ref{thm:bias} is that the score estimation bias depends on score and uncertainty. For a given model score, different samples can correspond to different true positivity rates based on uncertainty level, opening an opportunity to improve the quality of the decision boundary by considering both score and uncertainty. However, a direct adjustment of model score based on Theorem \ref{thm:bias} is not feasible or effective since the precise nature of distributional difference between test and train settings might not be known. 
% This is fairly common in large-scale real-life applications where legacy blackbox models are used for downstream prediction tasks or when there is  temporal drift. 
Even when there is information on differential sampling rate used in training, the class-conditional densities learned from sampled distributions tend to be different from the original distribution especially over sparse regions. 


==> sections/analysis_old.tex <==
We begin with a review of  Posterior Network followed by a theoretical analysis of score estimation bias.\\ 
%We begin with a review of preliminaries on uncertainty estimation and posterior networks followed by theoretical analysis of score estimation bias.
%\subsection{Preliminaries and Notation}
\noindent{\bf Notation.} Let $\x$ denote an input instance and $y$ the corresponding target label that takes values from the set of class labels $\cC =\{ 0, 1 \}$ with $c$ denoting the index over the labels.   Further, let  $\cD_{train}$ denote the data used for training, $\theta, \phi$ the model parameters and $\z= \z(\x)$ the output representation from the model. We use $\pr(\cdot)$ to denote probability and $[i]_{lb}^{ub}$ to denote an integer index taking values in $[lb, ub]$.

\subsection{Background: Posterior Network}
Posterior Network \citep{posterior_network} %provides a mechanism to 
estimates a closed-form posterior distribution over predicted class probabilities for any new input sample via density estimation. In particular, posterior networks comprise two components: a) an encoder network $f_{\theta}$ that maps potentially high dimensional input instance $\x$ to a low dimensional latent encoding %$\z=\z(\x)$ % 
$\z$ amenable for density estimation, and  b) a normalizing flow parameterized by $\phi$ for learning the normalized class-wise density functions $\pr(\z | c; \phi), ~ \forall c \in \cC$.  Since both the encoder network  and the normalizing flow are fully differentiable, their parameters $\theta, \phi$ are  jointly learned so as to optimize a free-energy like loss function that combines uncertainty cross-entropy loss ~\citep{uce} with the entropy of the posterior distribution over the class labels.

%SM: Should we add the objective function expression ?
In the case of binary classification, the posterior distribution over the class probabilities for an input point takes the form of a Beta distribution. For a given data sample, the parameters of the Beta distribution are estimated by combining the prior with pseudo-counts generated based on the learned normalized densities and observed class counts. Specifically,  denoting the prior and observed counts for the class $c \in \cC$ by $\beta_c^{prior}$ and $N_c$, the posterior distribution of the predicted class probabilities (also referred to as the epistemic distribution) for the point $\x$ is given by 
\begin{equation}
q(\x)=  \mbox{Beta}( \alpha_1(\x),\alpha_0(\x) )
\end{equation}
where $\alpha_c(\x)= \beta_c^{prior} + \beta_c(\x)$   and $\beta_c(\x) = N_c \pr(\z(\x) | c; \phi),~ \forall c  \in {\cal C}$.  The model score $s(\x)$ for positive class is given by 
\begin{equation}
s(\x) =  \frac{ \beta_1^{prior} +  \beta_1(\x)} { \sum_{c=0,1} [\beta_c^{prior} +  \beta_c(\x)]}  =  \frac{\alpha_1(\x)}{\alpha_1(\x) + \alpha_0(\x)} 
\end{equation}
The model uncertainty $u(\x)$ for $\x$ is given by the entropy of the epistemic distribution 
$H(q(\x))$.  Since $q(\x)$ is a Beta distribution, for the same score, i.e., ratio of $\alpha_1(\x)$ and $\alpha_0(\x)$, the uncertainty is higher when $\sum_{c \in \cC} \alpha_c(\x)$ is lower.

\subsection{Analysis of Estimation Bias}
%Estimation bias is defined as the difference between the model score and test positivity rate. 
Let us consider the case where the negative class is uniformly sampled during training at a different rate $\frac{1}{\tau}$ compared to the positive class\footnote{Note that $\tau >1 $ is the case where the negatives are undersampled while $\tau <1$ is the case of oversampling negative class.}. 
%From Bayes rule, the  positivity rate at $\x$ in the test dataset is  given by
%$$\pr(y=1|\x) =  \frac { \pr_{test}(y=1) \pr(\x | y=1)} {  \sum_{c=0,1} \pr_{test}(y=c) \pr(\x |y=c) }.$$
To keep the analysis tractable, we make an assumption about the model expressivity, i.e., the encoder network and normalizing flow accurately model the class-conditional distributions, and derive a closed  analytic form for the estimation bias, i.e., the difference between model score and test positivity rate. 

\noindent {\bf Assumption 2.1}  (Model Expressivity)  $\pr(\x |y=c)  \simeq \pr(\z(\x) | y=c ; \phi)$. \\


\begin{theorem} 
Under Assumption 2.1 with negative class undersampled at the rate $\frac{1}{\tau}$ during training, the estimation bias in the model score for the positive class  from Posterior Network at  $\x$  is given by
$$ \frac{e(s) +f(s)\gamma(\x)}{g(s)+h(s)\gamma(\x)}, $$ 
where $s=s(\x)$ denotes the model score and 
 \begin{itemize}
\item  $\omega =\frac{\beta_1^{prior}}{\beta_1^{prior} + \beta_0^{prior}}$ denotes the positive prior ratio,  
\item $\gamma(\x)  =  \frac{\beta_1^{prior} + \beta_0^{prior}} {\beta_1(x) + \beta_0(x)}$  denotes the relative strength of priors to evidence
\item $e(s) = s(1-s)(\tau-1) $; $~~f(s) = (1 + s(\tau - 1))(w-s)$
\item $g(s) = \tau - s(\tau-1)$; $~~h(s) = (\tau -1)(w-s) $.
\end{itemize}
\label{thm:bias}
\vspace{-2mm}
\end{theorem}


\proofsketch
Using Assumption 2.1 and adjusting for the differential sampling, we obtain test positivity rate at $\x$ as  
\begin{eqnarray*}
\pr(y=1|\x) &=&  \frac { \pr_{test}(y=1) \pr(\z(\x) | y=1)} {  \sum_{c=0,1} \pr_{test}(y=c) \pr(\z(\x) |y=c) } \\
&=& \frac{ \beta_1(\x) } { \beta_1(\x) + \tau \beta_0(\x)} 
\end{eqnarray*}
Expressing the above using $\omega$ and $\gamma(\x)$ and considering the difference
w.r.t. 
%relative to
the model score $s(\x)$ yields the result.
\qed

%SM: Do we need this?
% Below are a few observations on the above result

\noindent {\bf Interpretation of $\gamma(\x)$.}  Note that $\sum_c {\alpha_c(\x)}  =  [\sum_c \beta^{prior}_c ] (1 + \frac{1}{\gamma(\x)})$.  Since for a fixed score,  $\sum_c{\alpha_c(\x)}$  is inversely correlated to uncertainty $H(q(\x))$, we observe that $\gamma(\x)$ is positively correlated with $H(q(\x))$.

\noindent  {\bf No differential sampling $(\tau =1)$}. In this case, $e(s)=h(s)=0$,  $g(s)=1$ and $f(s)=(\omega-s)$. The estimation bias is given by $(\omega -s(\x))\gamma(\x)$. Essentially, since the model scores are estimated by combining the priors and the evidence, the model score differs from the empirical positivity rate in the direction of the class prior, i.e. there is overestimation in the lower score range $(\omega >s(\x))$ and the opposite is true when $(\omega < s(\x))$.  The extent of the bias depends on the relative strengths of the prior and the evidence  denoted by $\gamma(\x)$, which is correlated with uncertainty. 

\noindent  {\bf General case $(\tau > 1)$.} Here the behavior of the bias can be viewed as a combination of (i) the gap between model score and positivity rate in the train set, (ii) the gap between the positivity rate in the train and test set due to differential sampling. While the first component is similar to the case $\tau=1$ and results in over and under estimation in different score regions, the second component results in  overestimation across the entire score range with the extent of bias increasing with $\tau$.  Fig. ~\ref{fig:biasanalysis} shows the expected positivity rate for a few different choices of $\gamma(\x)$ and a fixed choice of $\omega=0.5$ and $\tau=10$. We validate this behavior by comparison with empirical observations in Section \ref{sec:experiment}. It can be shown that for a fixed choice of score, the estimation bias has an increasing or decreasing trend with respect to $\gamma(\x)$  (and thereby uncertainty) depending on whether $(s(\x)  <\omega)$ or $(s(\x) > \omega)$ (Corollary \ref{thm:fixedscore}).  However, for a fixed choice of uncertainty $\gamma(\x)$, the true positivity rate is monotonically increasing in the score 
but the valid score range is limited to $[\frac{ \omega\gamma(x)} {1+ \gamma(x)}, ~ \frac{ 1+ \omega\gamma(x)} {1+ \gamma(x)} ]$ due to effect of the prior as can be seen in Fig. ~\ref{fig:biasanalysis} (Corollary \ref{thm:fixedunc}). 

% \begin{figure}[t]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{sections/results/bias_analysis_simul.pdf}}
% \caption{Simulated estimated bias for different values of $\gamma$, for fixed values of $\tau=10$ and $\omega=0.5$}
% \label{fig:biasanalysis}
% \end{center}
% \vskip -0.2in
% \end{figure}

\begin{wrapfigure}{l}{0.5\textwidth}
% \hfill
\subfigure[]{\includegraphics[width=0.47\linewidth]{images/teaser/simul/Picture 21.pdf}}
\hfill
\subfigure[]{\includegraphics[width=0.4\linewidth]{images/teaser/simul/Picture 22.pdf}}
% \hfill
\vspace{-3mm}
\caption{\footnotesize (a) Positivity rate vs. model score for $\omega=0.5,~\tau=10$ and a few choices of $\gamma(\x)$ as per Theorem \ref{thm:bias}. (b) Positivity rate for different model 
score and uncertainty ranges on synthetic data.}
\label{fig:biasanalysis}
%\vspace{-6mm}
\end{wrapfigure}


% \begin{figure}[!htbp]
% \subfloat{%
%   \includegraphics[clip,width=0.8\columnwidth, height=4.5cm]{images/teaser/simul/positivity_analysis_simul_redo.pdf}%
% }
% \subfloat{%
%   \includegraphics[clip,width=0.8\columnwidth, height=4.5cm]{images/teaser/simul/bias_analysis_simul_redo.pdf}%
% }
% % \subfloat{%
% %   \includegraphics[clip,width=0.9\columnwidth]{images/teaser/mnist/hm_mnist_teaser_db.png}%
% % }
% % \vspace{-5mm}
% \caption{The plots demonstrate the relation between model score's level of over-estimation and the uncertainty range within which the samples lie, because of the differential sampling of negative class in train and test data. The heatmap plots the empirical positivity rate with different score and uncertainty ranges. Our proposed approach (red bar) results in incremental recall as compared to vanilla score based threshold (blue)}
% \label{fig:teaser-results}
% \end{figure}
The primary takeaway from Theorem \ref{thm:bias} is that the score estimation bias has a dependence on both score and uncertainty. Since it is possible that a model score can correspond to different actual positivity rates based on uncertainty level, we have an opportunity to improve the quality of the decision boundary by considering both score and uncertainty. However, a straightforward adjustment of the model score based on Theorem \ref{thm:bias} is often not feasible or effective since the precise nature of distributional difference between test and train settings might not be known. This is fairly common in large-scale real-life applications where legacy blackbox models are used for downstream prediction tasks or when there is  temporal drift. Even when there is information on the  differential sampling rate used in training, in practice, the class-conditional densities learned from the actual sampled distributions tend to be different from that from the original distribution especially over sparse regions. 


\begin{comment}
%SM: absorb this in related work
The uncertainty of the overall prediction can be computed as a hierarchical evaluation with contributions from each of the factors in the equation below~\citep{prior_network}:
\begin{center}
    \begin{equation}
        \pr(y | \x, \cD) = \int{\int{\underbrace{\pr(y|\z)}_{\text{data}}\underbrace{\pr(\z|\x, \phi)}_{\text{distributional}}\underbrace{\pr(\phi, \cD)}_{\text{model}} d\z d\phi}}
    \end{equation}
\end{center}

In particular, there are three contributing factors: a) {\em model uncertainty} associated with estimation of the model parameters $\phi$ from the training data $\cD$,  b) {\em distributional uncertainty} which corresponds to the variance in how a new input instance $\x$ is mapped to its output representation $\z$, which in turn depends on whether $\x$ is in a well-observed space (i.e., sufficient samples similar to $\x \in \cD$) or out-of-distribution, and c)  {\em data uncertainty} that arises from the inherent ambiguity in the target label $y$, which can be large even when $\x$ is in a well-observed region.  Typically, the first two factors are viewed as contributing to epistemic uncertainty while the last one is viewed as aleatoric uncertainty. 
\end{comment}
